OrchestRAN: Network Automation through Orchestrated Intelligence in the Open RAN

The next generation of cellular networks will be characterized by softwarized, open, and disaggregated architectures exposing analytics and control knobs to enable network intelligence. How to realize this vision, however, is largely an open problem. In this paper, we take a decisive step forward by presenting and prototyping OrchestRAN, a novel orchestration framework that embraces and builds upon the Open RAN paradigm to provide a practical solution to these challenges. OrchestRAN has been designed to execute in the non-real-time RAN Intelligent Controller (RIC) and allows Network Operators (NOs) to specify high-level control/inference objectives (i.e., adapt scheduling, and forecast capacity in near-real-time for a set of base stations in Downtown New York). OrchestRAN automatically computes the optimal set of data-driven algorithms and their execution location to achieve intents specified by the NOs while meeting the desired timing requirements. We show that the problem of orchestrating intelligence in Open RAN is NP-hard, and design low-complexity solutions to support real-world applications. We prototype OrchestRAN and test it at scale on Colosseum. Our experimental results on a network with 7 base stations and 42 users demonstrate that OrchestRAN is able to instantiate data-driven services on demand with minimal control overhead and latency.

==> journal_extension/dump_file.tex <==
\textbf{We can implement the following extensions:}
\begin{itemize}
    \item We only consider resources in terms of computation/storage and do not consider the case that all models in the same place might result in high overhead and congestion. We can model this in terms of bandwidth and should also affect the latency constraint as well as the constrained resource constraint. This should appear somewhere in $b_{d,d'}$, for example we could make it $b_{d,d'}(\mathbf{x})$ that is a decreasing function in the number of models running on a device and requiring a specific input. However, keep in mind that data might flow through nodes that are not just $d$ or $d'$ (e.g., the non-real-time RIC might get data from any node, but it has to go through many others in between;
    \item 
\end{itemize}

\subsection{Extending bandwidth model}

In theory, available bandwidth increases as we get close to the cloud where optical links with higher capacity are used to link network components. At the same time, if we deploy many models in the RIC, we also increase the amount of data traversing the network to reach the desired destination (e.g., where models are executed). For this reason, using a static value $b_{d',d''}$ to model the available bandwidth between two nodes might not be accurate enough to capture congestion at the different portions of the graph. For this reason, we might want to consider a load-based bandwidth model that account for how mush traffic flows at specific locations of the network. 

For each $(i,f,d,d')$, let $F^{i,f,d}_{d'}$ be an indicator variable defined as 
\begin{equation}
    F^{i,f,d}_{d'} = \sum_{m\in\mods} \sum_{k=1}^{C_{m,d'}} x^{i,f,d}_{m,k,d'} \chi_{i,f,d}
\end{equation}
\noindent
where $\chi_{i,f,d}\in\{0,1\}$ such that $\chi_{i,f,d}=1$ if and only if $|\devs_{i,f,d}| > 0$, i.e., there is at least one data flow to gather data from devices. Here we assume that gathering data from other models is negligible as model outputs have very limited size. 

Let $r^{d,d'}_{d''}\in\{0,1\}$ indicate whether or not the traffic flowing from $d$ to $d'$ traverses the same network node where element $d''$ is located (e.g., the same router/switch to whom node $d''$ is connected to). For example, $r^(d,d')_{d''}=1$ means that the traffic flowing from $d$ to $d'$ goes through a router that is also connected to $d''$. The total number $N_{d''}$ of flows traversing the same network node $d''$ can be computed as follows:
\begin{equation}
    N_{d''}(\mathbf{x}) = \sum_{i\in\reqs} \sum_{d\in\devs}\sum_{f\in\devs_{i,d}} \sum_{d'\in\devs} F^{i,f,d}_{d'} r^{d,d'}_{d''} 
\end{equation}

In this way, the bandwidth $b_{d',d''}$ can be formulated as a function of $\mathbf{x}$ as follows:
\begin{equation}
    b_{d',d''}(\mathbf{x}) = \frac{b_{d',d''}}{N_{d''}(\mathbf{x})} 
\end{equation}

This model is indeed not the most accurate, but captures eventual congestion or processing delay due to moving large amount of data from the edge to the cloud. Note that this should appear in the above constraints. Those are respectively linear and quadratic, this formulation will make them quadratic and cubic (good luck with that). 

% \subsection{Changing the utility function}

% In the above formulation we are assuming that all requests can be accommodated somehow. However, this might not be the case in highly resource constrained networks or latency constraints that are too stringent. In these cases, rather then minimizing the total number of instances in the network, we can maximize the number of satisfied requests. This can be achieved by introducing an indicator variable $y_i\in\{0,1\}$ such that $y_i = 1$ means we are satisfying request $i$, i.e., we instantiate all requested functionalities where they are needed and comply with minimum performance requirements and maximum tolerable latency. In this case, we need to reformulate constraint \eqref{eq:con1} as follows:
% \begin{equation}
%     \sum_{m\in\mods}\sigma_{m,f} \sum_{d'\in\devs} \sum_{k=1}^{C_{m,d'}} x^{i,f,d}_{m,k,d'} \leq \tau_{i,f,d} \label{eq:con1:updated}
% \end{equation}
% \noindent
% and add the following constraint
% \begin{equation}
%      \sum_{d\in\devs}\sum_{f\in\funcs_{i,d}} \sum_{m\in\mods}\sigma_{m,f} \sum_{d'\in\devs} \sum_{k=1}^{C_{m,d'}} x^{i,f,d}_{m,k,d'} = y_i \sum_{d\in\devs}  |\funcs_{i,d}|
% \end{equation}

% In this way, we can change the utility in $\max_{\mathbf{x}} \sum_{i\in\reqs} y_i v_i$, where $v_i$ represents the value (e.g., monetary or priority) of request $i$.

\section{Things to discuss}

\begin{enumerate}
    \item Which utility function do we want to maximize? Are we ok with minimizing the number of instances? Realistically, the only aspect that could make a request unfeasible is related to the lack of data and/or too much latency. Ideally, it might make sense to max the number of requests that are accepted, this might result in many non-shared models, but as soon as we start increasing the number of requests, we will experience higher sharing ratio. It might be not a bad idea to use the max(num reqs) utility;
    \item Do we want to consider an allocation-dependent bandwidth model? This would be very cool, but would make the problem even more complex than the current formulation. This would result in some kind of routing problem embedded in the instantiation problem. Not cool, not cool.
    \item We should define examples of $\tin_m$, to clarify how these could translate into functionalities. So far, it is not really clear, we should provide practical examples, especially if those functionalities relate to forecasting and classification and must be fed to another model.
    \item how do we deal with inputs of the same type but different size?
\end{enumerate}


% original equation
\begin{figure*}\footnotesize
\begin{align}
    \Delta^\mathrm{D}_{i,f,d}(\mathbf{x}) &= \sum_{m\in\mods} \sigma_{m,f} \sum_{d'\in\devs} \sum_{k=1}^{C_{md'}} x^{i,f,d}_{m,k,d'} \sum_{d''\in\devs^{\mathrm{IN}}_{i,f,d}} \left(\frac{s^\mathrm{D}_{\tin_m}}{b_{d',d''} |\devs^{\mathrm{IN}}_{i,f,d}|} + T_{d',d''} \right) \label{eq:delta_d}\\
    \Delta^\mathrm{M}_{i,f,d}(\mathbf{x}) &= \sum_{m\in\mods} \sigma_{m,f} \sum_{d'\in\devs} \sum_{k=1}^{C_{m,d'}} x^{i,f,d}_{m,k,d'} \left[ \sum_{d''\in\devs} c_{d',d''} \sum_{f'\in\funcs_{\tin_m}\cap\funcs_{i,d}\setminus\{f\}} \sum_{m'\in\mods_{\tin_m}\setminus\{m\}} \sigma_{m',f'} \sum_{k'=1}^{C_{m',d''}} x^{i,f',d}_{m',k',d''} \left( \frac{s^\mathrm{M}_{\tin_m}}{b_{d',d''} } + T_{d',d''} \right) \right] \label{eq:delta_m} \\
    \Delta^{EXEC}_{i,f,d}(\mathbf{x}) &= \sum_{m\in\mods}\sigma_{m,f} \sum_{d'\in\devs} \sum_{k=1}^{C_{m,d'}} x^{i,f,d}_{m,k,d'} \left[T^{exec}_{m,d'} + \lambda_{m,d'} \left(\sum_{i'\in\reqs} \sum_{d''\in\devs} \sum_{f'\in\funcs} x^{i',f',d''}_{m,k,d'} - 1\right) \right] \label{eq:execution}
    \end{align}
    \hrulefill
\end{figure*}

\subsection{Providing proper input}

As mentioned before, each model $m$ requires a specific type of input $\tin_m$. As a consequence, when instantiating a model on any node $d$, we must ensure that such input is available at $d$. As mentioned before, inputs can be generated by both nodes (e.g., throughput and channel measurements) and ML/AI models (e.g., predictions and classification outputs). 

In the former case, for any device $d$ and data type $t\in\types^\mathrm{D}$, let $\alpha_{d,t}\in\{0,1\}$ indicate whether or not device $d$ has access to data type $t$. Specifically, $\alpha_{d,t}=1$ indicates that node $d$ has direct access to data of type $t$, $\alpha_{d,t}=0$ otherwise. 
In the case of data generated by ML/AI models, for any $t\in\types^\mathrm{M}$, we define $\funcs_t\subseteq\funcs$ as the subset of functionalities that produce output $t$. Specifically, if $f\in\funcs_t$, then any model such that $m\in\mods_t$ satisfies $\funcs_m\cap\funcs_t \neq \emptyset$. Without loss of generality, we assume that $|\funcs_t \cap \funcs_m| \leq 1$. That is, for each output data type $t$, there is at most one functionality that, when executed by a ML/AI model,  provides that type of output.
% Here we assume that specific output data types are offered by models that provide specific functionalities. For example, a data type $t\in\types^\mathrm{M}$ representing forecast capacity can be provided by models that execute a specific function $f$ offering prediction of time series.

For each model $m\in\mods$, let $z_m$ be defined as follows:
\begin{align}
        z_m =&  \begin{cases}
                        1 \hspace{2cm} \mbox{if}~ \tin_m \in \types^\mathrm{D} \\
                        0 \hspace{2cm} \mbox{if}~ \tin_m \in \types^\mathrm{M} \\
                        0.5 \hspace{1.75cm} \mbox{if}~ \tin_m \in \types^\mathrm{DM}
                    \end{cases}        
\end{align}

Accordingly, to instantiate model $m$ on device $d$ we must satisfy the following constraint:
\begin{align}
    & x^{i,f,d}_{m,k,d'} \leq z_m \frac{1}{|\devs^{\mathrm{IN}}_{i,f,d}|}\sum_{d''\in\devs^{\mathrm{IN}}_{i,f,d}} c_{d',d''} \alpha_{d',\tin_m} \nonumber \\
    & + (1-z_m) \sum_{d''\in\devs} c_{d',d''} \sum_{f'\in\funcs_{\tin_m}\cap\funcs_{i,d}\setminus\{f\}} \nonumber \\
    & \sum_{m'\in\mods_{\tin_m}} \sigma_{m',f'} \sum_{k'=1}^{C_{m',d''}} x^{i,f',d}_{m',k',d''} \label{eq:con2}
\end{align}

For each control request $i$, the first term in the right part of \eqref{eq:con2} guarantees that a model is instantiated at network nodes that have access to data generated by nodes in $\devs^{\mathrm{IN}_i}$. Note that $\sum_{d''\in\devs^{\mathrm{IN}}_{i,f,d}} c_{d',d''} \alpha_{d',\tin_m} \leq |\devs^{\mathrm{IN}}_{i,f,d}|$. Therefore, when any of the selected models cannot be fed with the requested input data, we obtain $\sum_{d''\in\devs^{\mathrm{IN}}_{i,f,d}} c_{d',d''} \alpha_{d',\tin_m} /  |\devs^{\mathrm{IN}}_{i,f,d}| < 1$ which, due to the binary constraint on $x^{i,f,d}_{m,k,d'}$, implies $x^{i,f,d}_{m,k,d'}=0$. 
We consider the case where the input type of a model is different from the output type of the model itself, i.e.,  $\funcs_{\tin_m} \cap \funcs_m = \emptyset$.\footnote{This assumption does not exclude the case of forecasting applications where input data (e.g., throughput or latency measurements) is converted into a forecast of the same metric. In this case, it is worth noticing that although both input and output represent the same metrics (e.g., throughput or latency), they differ in that the former is a data type representing actual measurements, while the latter represents a prediction of future events, i.e., the data type is different.} We also assume that $|\funcs_{\tin_m} \cap \funcs_{i,d} \setminus \{f\}| \leq 1$. That is, (i) a model $m$ providing functionality $f$ and requiring input of type $\funcs_{\tin_m}$ cannot be used to generate its own input of type $\tin_m$, but should rely upon another functionality $f'\neq f$ provided by another model; and (ii)
the functionality $f'$ producing input of type $\funcs_{\tin_m}$ for model $m$ must be selected among those already included in the set of requested functionalities $\funcs_{i,d}$.
Under these assumptions, and under constraint \eqref{eq:con1}, the term on the right hand side of \eqref{eq:con2} is either 0 or 1. 

\subsection{ML/AI catalog and functionalities} \label{sec:catalog}

We consider the case where all the data-driven solutions that can be instantiated in the network are stored in a ML/AI catalog. According to O-RAN specifications, such models are already pre-trained offline in the non-RT RIC \cite{}, and have been already tested and validated to ensure their effectiveness and reliability.

Let $\mods$ be the set of data-driven models in the ML/AI catalog, and let and $\funcs$ represent the entire set of possible control/inference functionalities (e.g., scheduling, beamforming, capacity forecasting, handover prediction, to name a few) offered by the models in the ML/AI catalogue. 
For each model $m\in\mods$, $\funcs_m \subseteq \funcs$ represents the subset of functionalities offered by model $m$. Accordingly, we define a binary variable $\sigma_{m,f}\in\{0,1\}$ such that $\sigma_{m,f}=1$ when functionality $f\in\funcs_m$, $\sigma_{m,f}=0$ otherwise. 

It is worth mentioning that, although two models $m'$ and $m''$ can provide the same functionalities, i.e., $\funcs_{m'} = \funcs_{m'}$, they might differ one another in terms of model size, required inputs and offered outputs. For example, both models $m'$ and $m''$ can provide data-driven control of scheduling operations via DRL. However, model $m'$ might compute scheduling strategies based upon throughput and latency measurements individually reported by a set of DUs, while the decision making of model $m''$ relies upon the status of the transmission queues at each DU only. 

To model the diversity of the ML/AI catalog in terms of resources required to instantiate and execute a ML/AI model, we use $\rho^\xi_m$ to indicate the amount of resources of type $\xi$ required to instantiate and execute model $m$. Similarly, let $\types$ be the set of possible input (output) types that each model requires (produces). For each model $m\in\mods$, let $\tin_m\in\types$ be the type of input required by the model. Since models are diverse, we consider the following three cases: (i) the input contains data that can be measured and collected by nodes of the network (e.g., throughput, transmission buffer size, IQ samples); (ii) the input to the model corresponds to the output produces by other models (e.g., capacity forecasting and scheduling policies computed by DRL agents); and (iii) a combination of the two former cases. We define $\types^\mathrm{D}$, $\types^\mathrm{M}$ and $\types^\mathrm{DM}$ to distinguish between the three above cases, e.g., $\tin_m\in\types^\mathrm{D}$ means that model $m$ requires input that can be gathered by devices only. 
Similarly, we let $\tout$ be the set of all output data types while $\tout_m$ represents the set of output types produced by model $m$. Indeed, each model can produce several types of outputs. For example, the same model can used to forecast capacity and, at the same time, compute optimal scheduling policies. 
For each data type $t\in\types$, we identify $\mods_t\subseteq\mods$ as the set of models whose output contains type $t$. Specifically, $\mods_t = \{m\in\mods : t \in \tout_m\}$.

\subsubsection{Modeling execution time} For any orchestration strategy $\mathbf{x}$ and tuple $(i,f,d)$, the execution time $\Delta^{EXEC}_{i,f,d}(\mathbf{x})$ is defined by \eqref{eq:execution}, where $T^{exec}_m$ represents the time needed to execute model $m$ on device $d'$ (i.e., the time needed to convert an input into an output), and $\lambda_{m,d}$ is a parameter that we will describe in the following and is used to model the impact of model sharing on the execution time of a shared model.

\textbf{\color{red}[We might want to remove this latency related to model sharing to keep the problem non-linear]}

As discussed in Section \ref{sec:orchestration}, the same model can be shared across multiple requests to reduce the impact on resource utilization. However, sharing might result in increased processing latency as inputs from multiple requests are processed sequentially, which results in a waiting queue where outstanding requests wait to be fed to the ML/AI model. As a consequence, the higher the number of requests sharing the same model, the higher the latency each request will experience. While such a latency might be negligible in slowly varying scenarios and non-real-time applications, it might hinder the effectiveness of real-time applications involving, for example, URLLC traffic. For this reason, model sharing should always be encouraged but only in those cases where it does not affect compliance with SLAs.
To model this performance degradation, we use a congestion-like formulation (frequently used to model performance loss due to link congestion in routing problems~\cite{}) where the negative effect of model sharing is expressed as a decreasing linear function of the number of requests sharing the same model. The slope of the function is represented by the parameter $\lambda_{m,d}$.
 
With the above formulation at hand, we are now able to formulate the constraint which ensures that the timing constraint $\delta_{i,f,d}$ is satisfied. Specifically, any orchestration policy $\mathbf{x}$ must satisfy the following constraint:

\begin{equation}
  \Delta_{i,f,d}(\mathbf{x}) + \Delta^{EXEC}_{i,f,d}(\mathbf{x}) \leq \delta_{i,f,d} \tau_{i,f,d} \label{eq:latency_tot}
\end{equation}


\begin{figure}[h]
\begin{centering}
    \includegraphics[width=\columnwidth]{figs/datageneration.pdf}
    \caption{Dataset generation and training pipelines and their integration with the experimental testbeds described in Task 4.}
    \label{fig:emulation}
\end{centering}
\end{figure}

% # this was in Assigning ml/ai models to contorl requests
A request $i$ is said to be satisfied (i.e., $y_i=1$) if and only if all functionalities in $\funcs_i$ are provided at desired locations. For any request $i$, this requirement can be formalized via the following constraint \textbf{\color{red}[i don't think we need this]}
\begin{equation}
     \sum_{d\in\devs}\sum_{f\in\funcs_{i,d}} \sum_{m\in\mods}\sigma_{m,f} \sum_{d'\in\devs} \sum_{k=1}^{C_{m,d'}} c_{d,d'} x^{i,f,d}_{m,k,d'} = y_i \sum_{d\in\devs}  |\funcs_{i,d}| \label{eq:con1:add}
\end{equation}

==> journal_extension/old_sec_3_4.tex <==

\section{\name Overview}

The system architecture of \name and its core building blocks are illustrated in Fig. \ref{fig:system}.

\name features a \textit{ML/AI Catalog} (described in detail in Section \ref{sec:catalog}) that stores all data-driven solutions that can be instantiated in the network. An \textit{Infrastructure Abstraction} module allows \name to gain relevant information on the underlying physical infrastructure such as available resources, cell coverage, deployment location of \glspl{ric} and \gls{ran} components (Section \ref{sec:infra}). 

In \name, \glspl{to} specify their intent by submitting a control request (Step I). This includes the set of functionalities they want to deploy (e.g., network slicing, beamforming and scheduling control, capacity forecasting, among others), the nodes of the network where such functionalities are required (e.g., a specific \gls{ric} or \gls{du}) to execute as well as the desired time scale (e.g., \nonrt, \nearrt, \rt). Requests are gathered by the \textit{Request Collector} (Step II and Section \ref{sec:control_request}) and fed to the \textit{Orchestration Engine} (Step III and Section \ref{sec:orchestration_engine}) which: (i) accesses the ML/AI catalog and, thanks to the information obtained via the Infrastructure Abstraction module, computes the optimal orchestration policy specifying which ML/AI models should be instantiated and where to accommodate \glspl{to} requests; (ii) automatically creates containers in the form of rApps, xApps and dApps that embed the selected ML/AI models and already subscribes each container to the nodes of the \gls{ran} whose data will be fed to the embedded ML/AI models; and (iii) automatically dispatches and instantiates the generated containers at the locations determined by the Orchestration Engine. 

\section{Building blocks and system model} \label{sec:system}

The objective of this section is illustrate \name building blocks, the considered system model and how it fits within the \oran disaggregated and softwarized vision. 

\subsection{The Infrastructure Abstraction module} \label{sec:infra}

The Infrastructure Abstraction module provides a high-level and abstract representation of the physical architecture. Following \oran specifications, the abstraction of the physical infrastructure is represented by the hierarchical structure in Fig. \ref{fig:system_split} (right) where the physical infrastructure is divided into $L=5$ separate logical groups: \nonrt \glspl{ric}, \nearrt \glspl{ric}, \glspl{cu}, \glspl{du} and \glspl{ru}. 

Each group contains a different number of nodes 
% (e.g., the number of \glspl{ru} is substantially larger than the number of non-RT \glspl{ric} in the network), 
that are physically deployed at different locations of the network. 
% However, it is worth mentioning that the models and algorithms presented in this article are general and can be easily extended to different values of $L$ and architectures.
% represents different network components executing diverse procedures, providing different functionalities and instantiated at different locations of the infrastructure. 
Let $\devs$ be the set of such nodes, and let $D=|\devs|$ be their number. Due to the hierarchical structure of the infrastructure, it is easy to notice that the number of \glspl{ru} is substantially larger than the number of \glspl{ric} in the network.
% In general, that can host and execute data-driven models. 
Therefore, the hierarchical relationships between nodes in the considered architecture can be represented via an undirected graph with a tree structure such as the one in Fig. \ref{fig:system_split} (right). Specifically, leaves represents nodes at the edge (e.g., \glspl{ru},\glspl{du},\glspl{cu}), while servers in the cloud hosting \glspl{ric} are represented by roots and branches of the graph. For any two devices $d'$ and $d''$ in $\devs$, we define a \textit{reachability indicator} $c_{d',d''}\in\{0,1\}$ such that $c_{d',d''}=1$ if device $d'$ is reachable from device $d''$ (e.g., there exist a communication link such that node $d'$ can forward data to node $d''$), $c_{d',d''}=0$ otherwise. 
Moreover, for each node $d\in\devs$, let $\rho^\xi_d$ be the total amount of resources of type $\xi\in\Xi$ dedicated to hosting and executing ML/AI models and their functionalities, where $\Xi$ represents the set of all resource types. Although we do not make any assumptions on the specific types of resources, practical examples include: number of CPUs, GPUs, as well as available disk storage and memory.  

It is worth mentioning that, although \glspl{ru},\glspl{du} and \glspl{cu} are logically separated entities, in some cases they might coexist on the same physical hardware and share the same resources. This case can be captured by considering a single logical node whose hierarchy level in the tree graph matches the hierarchy of the highest logical node in the group of co-located nodes. For example, a \gls{du} and \gls{ru} co-located at the same physical node will be represented as a leaf node with hierarchy level four (i.e., the hierarchy level of the \gls{du}).

\subsection{The ML/AI catalog} \label{sec:catalog}

In \name, the available data-driven solutions that can be instantiated in the network are stored in a \textit{ML/AI catalog}. Although our framework is general and supports both offline and online data-driven solutions, we specifically follow \oran specifications and requirements, which dictate that all models contained in the ML/AI catalog must have been already pre-trained offline in the \nonrt \gls{ric}~\cite{}, and have successfully passed validation tests to ensure their effectiveness and reliability once deployed on the field.

\begin{figure}[t]
\begin{centering}
    \includegraphics[width=0.7\columnwidth]{figs/system.pdf}
    % \vspace{-1.5cm}
    \caption{System design of \name and main procedures.}
    \label{fig:system}
\end{centering}
\end{figure}

Let $\mods$ be the set of models in the ML/AI catalog, and let $\funcs$ represent the entire set of possible control and inference functionalities (e.g., scheduling, beamforming, capacity forecasting, handover prediction, to name a few) offered by such models. The total number of ML/AI models in the catalog and functionalities are $M=|\mods|$ and $F=|\funcs|$, respectively.
For each model $m\in\mods$, $\funcs_m \subseteq \funcs$ represents the subset of functionalities offered by $m$. Accordingly, we define a binary variable $\sigma_{m,f}\in\{0,1\}$ such that $\sigma_{m,f}=1$ if $f\in\funcs_m$, $\sigma_{m,f}=0$ otherwise. 

It is worth mentioning that two models $m'$ and $m''$ providing the same functionalities, i.e., $\funcs_{m'} = \funcs_{m''}$ might differ in terms of model size as well as required inputs. For example, although two models $m'$ and $m''$ use \gls{drl} to control scheduling operations, model $m'$ might compute scheduling strategies based upon throughput and latency measurements individually reported by a set of \glspl{du}, while the decision making process of model $m''$ might rely upon the status of the transmission queues at each \gls{du} only. Similarly, the \gls{drl} agent of model $m'$ might use a deep architecture, while $m''$ might be using an agent with a shallower and lightweight architecture.

To model such diversity, we use $\rho^\xi_m$ to indicate the amount of resources of type $\xi\in\Xi$ required to instantiate and execute model $m$. Similarly, let $\types$ be the set of possible input types that each model requires. For each model $m\in\mods$, let $\tin_m\in\types$ be the type of input required by the model. Practical examples of input types that are relevant to \oran applications are throughput, transmission buffer size, IQ samples, network load, scheduling policies, bit error rate, among others.

Although virtualization and softwarization make it possible to easily instantiate software via containers on general purpose hardware, not all AI/ML models can execute everywhere. For example, if one of the functionalities offered by a model $m\in\mods$ is RF fingerprinting~\cite{}, where IQ samples received on the RF front-end are classified by a neural network to authenticate the transmitting device, model $m$ can execute only on those nodes where those IQ samples are actually available. Indeed, while IQ samples can be accessed in real-time at the \gls{ru}-level, they are unlikely to be available at \glspl{cu} and the \glspl{ric}. Indeed, transferring IQ samples from \glspl{ru} to the cloud requires high bandwidth as these samples are complex-valued numbers represented in double-precision floating point format, which inevitably results in high overhead and transmission latency. For this reason, we introduce a suitability indicator $\beta_{m,f,d}\in[0,1]$ which specifies how well a model $m$ is suited to provide a specific functionality $f\in\funcs$ when instantiated on node $d$. Values of $\beta_{m,f,d}$ closer to $1$ mean that the model is well-suited to execute at a specific location, while values closed to $0$ indicate that the model performs poorly due to the lack of input data at device $d$, or due to high computation latency that violates timing requirements (e.g., real-time) of that functionality. Although our model is general and does not target specific applications, it is reasonable to assume that $\beta_{m,f,d}\in\{0,1\}$, i.e., the model $m$ is suited to provide functionality $f$ on node $d$, or it is not in the majority of practical applications. Moreover, we introduce a performance score $\pi_{m,f}$ which describes the performance of the model with respect to function $f\in\funcs_m$. Possible performance metrics are model classification/forecasting accuracy, mean squared error, probability of false alarm, among others. For example, models for classification tasks will be characterized by their classification accuracy, while models for forecasting applications might be described by their mean squared error metric (i.e., the prediction accuracy).

It is worth mentioning that the same model can be instantiated on the same node multiple times to serve different network operators or classes of traffic. However, since each node has limited resources $\rho^\xi_d$ of type $\xi$, each node $d$ can support a maximum number $C_{m,d}=\min_{\xi\in\Xi} \left \{ \left \lfloor \frac{\rho^\xi_d}{\rho^\xi_m} \right \rfloor \right  \}$ of instances of model $m$,
% . Specifically,    
% \begin{equation}
    % C_{m,d} \leq \min_{\xi\in\Xi} \left \{ \left \lfloor \frac{\rho^\xi_d}{\rho^\xi_m} \right \rfloor \right  \}.
% \end{equation}
% \noindent
where $\lfloor \cdot \rfloor$ is the floor operator.  

\subsection{Request Collector} \label{sec:control_request}

\name allows network operators to submit control requests specifying which functionalities they require, where these should execute, as well as the desired performance and timing requirements.
The Request Collector module of \name is in charge of collecting such requests. Specifically, a control request $i$ is defined as a tuple $(\funcs_i,\boldsymbol{\pi}_i,\boldsymbol{\delta}_{i}, \devs^{\mathrm{IN}}_{i})$. Each element of the tuple is defined as follows:
\begin{itemize}[leftmargin=*]
    \item \textit{Functions and locations}: For each control request $i$, we define the set of control functionalities that must be instantiated on desired nodes of the infrastructure as $\funcs_i=(\funcs_{i,d})_{d\in\devs}$, with $\funcs_{i,d}\subseteq\funcs$. To indicate whether or not a control request $i$ requires functionality $f$ on node $d$, we define a binary indicator $\tau_{i,f,d}\in\{0,1\}$ such that $\tau_{i,f,d}=1$ if $f\in\funcs_{i,d}$, i.e., function $f$ is requested on node $d$, $\tau_{i,f,d}=0$ otherwise. We also define $\devs_i=\{d\in\devs: \sum_{f\in\funcs_i} \tau_{i,f,d} \geq 1\}$ as the subset of nodes of the network where functionalities $f\in\funcs_i$ should be offered;
    \item \textit{Performance requirements}: For any request $i$, $\boldsymbol{\pi}_i=(\pi_{i,f,d})_{d\in\devs_i, f\in\funcs_{i,d}}$ indicates minimum performance requirements that must be satisfied to accommodate control request $i$. For example, if $f$ is a beam detection functionality, $\pi_{i,f,d}$ can represent the minimum detection accuracy of the model. Similarly, in the case of capacity forecasting, a control request can specify a maximum tolerable \gls{mse} level. In general, we do not make any assumptions on the physical meaning of $\pi_{i,f,d}$ as it might differ from one functionality to the other. As we will show in Section \ref{sec:quality}, this parameter will be important to identify those ML/AI models and nodes that are suitable to accommodate request $i${\ifCompile\color{blue}. For example, if $\tau_{i,f,d}=1$ and $\sigma_{m,f}=1$ for a model $m\in\mods$, such model can be instantiated on device $d$ to deliver functionality $f$ requested by $i$ if and only if $m$ is suitable, that is $\beta_{m,f,d}\geq \pi_{i,f,d}$\fi};
    \item \textit{Timing requirements}: $\boldsymbol{\delta}_i=(\delta_{i,f,d})_{d\in\devs_i, f\in\funcs_{i,d}}$ represents the maximum latency request $i$ can tolerate to execute functionality $f$ on device $d$. Indeed, all functionalities could be executed at the \nonrt \gls{ric} which has full-knowledge of the entire network and can potentially control each network node. However, some functionalities might have strict latency requirements $\delta_{i,f,d}$ that make their execution at specific nodes of the network unpractical or inefficient{\ifCompile\color{blue}. For example, although instantiating a ML/AI model to execute beam prediction at the \nonrt \gls{ric} might be possible, it does not guarantee real-time response time as IQ samples and other data necessary to control the transmission (or reception) beams must travel from the \glspl{ru} throughout the entire network and reach the \nonrt \gls{ric}, which inevitably incur in high latency and violation of real-time requirements\fi};
    \item \textit{Data source}: for each control request $i$, the network operator also specifies the subset of nodes whose generated (or collected) data must be used to deliver functionality $f$ on node $d$. This set is defined as $\devs^{\mathrm{IN}}_{i}=(\devs^{\mathrm{IN}}_{i,f,d})_{d\in\devs_i, f\in\funcs_{i,d}}$, where $\devs^{\mathrm{IN}}_{i,f,d}\subseteq\devs$. This information is fundamental to ensure that each AI/ML model is fed with the proper data generated by the intended sources only {\ifCompile\color{blue}. For this reason, for any tuple $(i,f,d)$ we assume that $c_{d,d'}=1$ for all $d'\in\devs^{\mathrm{IN}}_{i,f,d}$, i.e., data collection from $\devs^{\mathrm{IN}}_{i,f,d}$ to node $d$ is always feasible. It is worth mentioning that ML/AI models are built to receive inputs in a specific format, but do not differentiate between different data sources as soon as the input format is satisfied. For this reason, it is important that specific functionalities process data generated by intended sources only. As an example, if an operator is interested in instantiating a ML/AI model to forecast the capacity of the traffic generated in a specific area of interest covered by nodes $\devs'\subseteq\devs$, such a model must process data generated by nodes in $\devs'$ only, and neglect any data generated by any other node $\devs'' \subseteq \devs \cap \devs'$.\fi}
\end{itemize}

In the following of this paper, we use $\reqs$ to represent the set of outstanding control requests with $I=|\reqs|$ being their number.

\subsection{The Orchestration Engine} \label{sec:orchestration_engine}

As shown in Fig.~\ref{fig:dispatch}, once the control requests are submitted to \name, 
% the next step consists in determining which requests can be accommodated and orchestrating the corresponding ML/AI models. This task is accomplished by 
the Orchestration Engine selects the most suitable models from the ML/AI catalog as well as the exact location where these model should execute (Step I). Then, \name embeds such models into containers (e.g., xApps, rApps) (Step II), which are then dispatched to the selected nodes (Step III) where they are fed with data coming from the \gls{ran} to execute their functionalities (Step IV). 

The selection of the most suited ML/AI models and their optimal execution location is performed by solving an optimization problem---i.e., the \textit{orchestration problem}, whose formulation and solutions will be discussed in detail in Sections \ref{sec:orchestration_problem} and \ref{sec:solutions}---which results in an \textit{orchestration policy}. This is then converted into a set of rApps, xApps and dApps that are dispatched and executed at the designed network nodes as discussed in the following. 

\begin{figure}[t]
\begin{centering}
    \includegraphics[width=\columnwidth]{figs/dispatch.pdf}
    \vspace{-1.5cm}
    \caption{Container creation and dispatchment procedures in \name with \oran E2-SM interface to collect data from relevant network nodes.}
    \label{fig:dispatch}
\end{centering}
\end{figure}

\subsubsection{Container creation}
%
% \textbf{[Here goes how we embed models inside containers]}
%
To seamlessly deploy the same ML model in each app category, we integrate two subsystems in the containers, which are automatically compiled from descriptive files upon instantiation. The first is the ML model itself, and the second is an app-specific \textit{connector}, a library that interfaces with the DU itself (dApps), the near-real-time \gls{ric} platform (xApps), and the non-real-time \gls{ric} (rApps). The connector takes care of pulling data and sending control information between the specific platform and the ML model.

\subsubsection{Instantiation and orchestration}
% \textbf{[here goes how we instantiate containers, subscribe models to nodes, send data via E2 SM (to get input) and use E2 to send control actions]}
%
After each optimization step, the orchestrator dispatches container creation commands to the proper endpoints, specifying the ML model to deploy and the input and output requirements of each container. If the container is deployed as an xApp, it automatically send an E2 subscription request to the nodes it needs to fetch input from. A pair of custom \glspl{sm} are then used to collect data and send control over E2. 

